The MUSE Extremely Deep Field: the Cosmic Web in Emission at High Redshift

We report the discovery of diffuse extended Ly-alpha emission from redshift 3.1 to 4.5, tracing cosmic web filaments on scales of 2.5-4 comoving Mpc. These structures have been observed in overdensities of Ly-alpha emitters in the MUSE Extremely Deep Field, a 140 hour deep MUSE observation located in the Hubble Ultra Deep Field. Among the 22 overdense regions identified, 5 are likely to harbor very extended Ly-alpha emission at high significance with an average surface brightness of $\mathrm{5 \times 10^{-20} erg s^{-1} cm^{-2} arcsec^{-2}}$. Remarkably, 70% of the total Ly-alpha luminosity from these filaments comes from beyond the circumgalactic medium of any identified Ly-alpha emitters. Fluorescent Ly-alpha emission powered by the cosmic UV background can only account for less than 34% of this emission at z$\approx$3 and for not more than 10% at higher redshift. We find that the bulk of this diffuse emission can be reproduced by the unresolved Ly-alpha emission of a large population of ultra low luminosity Ly-alpha emitters ($\mathrm{<10^{40} erg s^{-1}}$), provided that the faint end of the Ly-alpha luminosity function is steep ($\alpha \lessapprox -1.8$), it extends down to luminosities lower than $\mathrm{10^{38} - 10^{37} erg s^{-1}}$ and the clustering of these Ly-alpha emitters is significant (filling factor $< 1/6$). If these Ly-alpha emitters are powered by star formation, then this implies their luminosity function needs to extend down to star formation rates $\mathrm{< 10^{-4} M_\odot yr^{-1}}$. These observations provide the first detection of the cosmic web in Ly-alpha emission in typical filamentary environments and the first observational clue for the existence of a large population of ultra low luminosity Ly-alpha emitters at high redshift.

==> clustering.tex <==
% Clustering


\begin{figure*}[htbp]
\begin{center}
\includegraphics[width=0.9\paperwidth]{clustering.pdf}
\caption{Spatial clustering of LAE in groups. LAE are shown as red circle sized according to their \lya\ luminosity. The location of each group member is overlayed on the HST F775W grey scale image. The fields locations are shown as a grey circle (\mxdf) superimposed on a square (\udft). Group id and redshift are labbeled. Fields have the \mosaic\ size and orientation, i.e. 3 arcmin and -42\degree\ PA.
The grey line at the bottom of each image indicates the 5 Mpc comoving scale.
}
\label{fig:clustering}
\end{center}
\end{figure*}

We now investigate the spatial clustering of LAE in the overdensities. LAE spatial location for each group are displayed in Figure~\ref{fig:clustering}.

At first sight, LAEs do not seem to be randomly placed in the field, but rather aligned along some elongated structure (aka filaments) like in groups 1,2,10,12,16. In other case, e.g. group 14, one might interpret the shape as the crossing of 2 or 3 filaments. However the transverse field of view (5.7 - 7.4 Mpc depending of z) can capture only a fraction of the expected filament lengths and the line-of-sight width is large enough (5 Mpc) to possibly embrace more than one filament making the projected image difficult to interpret. 

To quantify this impression, we first test if these geometrical shapes can result from random placement. For each group we compare its actual 2D geometry with the figure obtained by random placement of the same number of points. We use the multi-dimensional version of the well known Kolmogorov-Smirnov test \citep{Fasano1987}. The KS2D test measure the probability of the two samples of points to result from the same distribution. We produce a large number of random fields (10,000) and measure their KS2D probability Pval (high value indicate that the 2 fields are statistically similar). The relative number of occurrence of e.g. Pval$>$0.95, will give us the probability of similarity of the 2 distribution of points. 

Note that the KS2D test is not invariant by translation or rotation. Pattern with perfect matching shape but translated will not result in Pval=1. Given that we are interested in the similarity of shape, for each produced pattern we measured the highest KS2D probability by systematically performing a combination of spatial offset and flip along the two axis.

This exercise demonstrate that the hypothesis of random location of LAEs can be rejected for all groups with a probability of $\mathrm{P > 1 - 10^{-4}}$.

The next step would be to identify the geometrical filamentary pattern in our LAEs distribution. Various methods have been developed to measure cosmic web patterns from galaxy cosmological simulations or large sky surveys (e.g \citealt{Santiago2020}, see also the review by \citealt{Libeskind2017}). However, these methods are not well adapted to our volume characteristics: i.e. a small transverse size plus a relative thickness along the line of sight.

We have therefore opted for an approach, similar to the one used to test random fields, but this time using geometrical points patterns resulting from numerical cosmological simulation of LAE groups with similar characteristics that our measured sample.

\todo{decription and results. one or 2 images of group, showing the best case from random and simulation with their probability} 


Narrow band \lae\ wide field surveys, follow-up by spectroscopic multi-object observations, have produced a wealth of information on LAE clustering and the large scale structure of galaxies at high z (e.g. \citealt{Francis2004, Matsuda2005, Zheng2016}). They cover a large volume: e.g. $\mathrm{200 \times 200 \times 80 \, Mpc^3}$ for the SILVERRUSH survey \citep{Ouchi2017, Shibuya2017}, at the expense of bright limiting luminosity (typically $\sim 10^{43}$\ergslum)
and sparse sampling (e.g. 179 LAE for the \citealt{Harikane2019} study, that is $\mathrm{5.6\,10^{-5} Mpc^{-1}}$).

With two order magnitude higher average density ($\mathrm{6.3\,10^{-3} Mpc^{-1}}$ at z=6), our study probe for the first time the large scale structure at high z with a much finer sampling. Thanks to this zoomed view of the cosmic web, we can resolve the filamentary structure in unprecedented detail. \todo{expand and link to next section}


 

==> local_uvb.tex <==
%\documentclass[usenatbib,fleqn]{article}
%\usepackage[pdftex]{graphicx}
%\usepackage{amsmath}
%\usepackage[latin1]{inputenc}
%\parindent0em
%\usepackage{natbib}
%\usepackage{subfigure}
%\usepackage[left=2.5cm,right=3.5cm,top=2cm]{geometry} 

%\newcommand{\lya}{Ly$\alpha~$} 
%\newcommand{\msun}{\ifmmode M_{\odot} \else M$_{\odot}$\fi}

\label{app:uvb}

Following \cite{Kakiichi2018}, we write the \hi photoionisation rate $\Gamma^{\rm LAE}_{HI} (r)$ due to \textit{local} ionising background, i.e. the ionising emission from a LAE, as:

\begin{equation}
\label{eq1}
\Gamma^{\rm LAE}_{HI} (r) = \frac{\alpha_{\rm g} \sigma_{\rm 912}}{\alpha_{\rm g}+3} \frac{\dot{N}^{\rm LAE}_{\rm ion}}{4 \pi r^2} e^{-r/\lambda_{\rm mfp}(z)}
\end{equation}

where $\alpha_{\rm g} \approx 2$ is the extreme UV ($> 13.6$ eV) spectral slope, $\sigma_{\rm 912}=6.35 \times 10^{-18}$ cm$^2$ is the \hi photoionisation cross-section at $912$ \AA, and $\lambda_{\rm mfp}(z) \approx 37[(1+z)/5]^{-5.4}$ is the mean free path of ionising photons (in pMpc) at a given redshift $z$ \citep{Worseck2014}. The ionising production rate due to the LAE can be expressed as : 
\begin{equation}
\label{eq2}
\dot{N}^{\rm LAE}_{\rm ion} = f_{\rm esc} \xi_{\rm ion} L_{\nu}^{\rm UV}\\
\end{equation}

The quantities in the right-hand term are defined as follows :

\begin{itemize}
\item $f_{\rm esc}$ is the fraction of ionising photons produced by the galaxy that escape from the CGM. We assume that typical $f_{\rm esc}$ values are $0.02-0.2$.

\item $\xi_{\rm ion}$ corresponds to the emission rate of hydrogen-ionizing photons per unit UV (1500A) luminosity density and is expressed in $[$erg$^-1$ Hz$]$. At $z=3-6$, log$\xi_{\rm ion}$ is estimated to range between $25.2$ and $25.7$ \citep{Robertson2013, Nakajima2018}.\\

\item $L_{\nu}^{\rm UV}$ is the UV luminosity density of the galaxy, usually evaluated at 1500 \AA. Given that our LAEs are not detected in the UV, we estimate the UV luminosity density $L_{\nu}^{\rm UV}$ from the SFR. Following \cite{Kennicutt1998}, we can write $L_{\nu}^{\rm UV} [\rm{erg s}^{-1} \rm{Hz}^{-1}] = \eta ({\rm SFR}/M_{\odot} \rm{yr}^{-1})$. For a Salpeter IMF, $\eta = 8 \times 10^{27}$  for solar metallicity and $\eta = 1.7 \times 10^{28}$ for $Z = 0.005 Z_\odot$ \citep{Robertson2013}.

\end{itemize}

We can rewrite Eq. \ref{eq2} as $\dot{N}^{\rm LAE}_{\rm ion} = <f_{\rm esc} \xi_{\rm ion} \eta> ({\rm SFR}/M_{\odot} \rm{yr}^{-1})$. Using the possible values of the model parameters mentioned above, $<f_{\rm esc} \xi_{\rm ion} \eta>$ is comprised between $2.5 \times 10^{51}$ and $1.7 \times 10^{53}$ $[\rm{s M}_{\odot}^{-1} \rm{yr}]$.  \\

Therefore, using this formalism, the \hi photoionisation rate induced by a LAE at a distance $r$ amounts to:
\begin{equation}
\label{eq4}
\Gamma^{\rm LAE}_{HI} (r) = 2.5 \times 10^{-18} \frac{<f_{\rm esc} \xi_{\rm ion} \eta> {\rm SFR}}{4 \pi r^2} e^{-r/\lambda_{\rm mfp}(z)}
\end{equation}

In order to estimate the local UV background in the filament due to all individual LAEs of the group, one can write an effective photoionisation rate, $\Gamma^{\rm eff}_{HI}$, as the sum of all galaxy contributions:

\begin{equation}
\label{eq5}
\Gamma^{\rm eff}_{HI} = \sum_{i} \Gamma^{\rm LAE,i}_{HI} (r_i) 
\end{equation}
where $r_i$ is the distance from each LAE to the filament. 



For each group we have derived a photo-ionization map using the location and SFR of each \laes.  We use the following parameters $f_{\rm esc} = 0.1$, $\xi_{\rm ion} = 10^{25.2}$ and  $\eta = 8 10^{27}$. We then compute $\Gamma_{\rm HI}^{\rm LAE}$ by taking the average value on the diffuse segmentation area. Values are reported in Table \ref{tab:uvb} section \ref{subsec:uvb}.

Note that for HST undetected LAE, we have used the following standard relation to estimate the SFR from the \lya\ luminosity:

\begin{equation}
\label{eq6}
{\rm SFR} = 9.1 10^{-43} L_{\lya} 
\end{equation}
where $L_{\lya}$ is the \lya\ luminosity in \ergslum.


%\clearpage

%Kakiichi et al. (2018)

%https://ui.adsabs.harvard.edu/abs/2018MNRAS.479...43K/abstract \\

%Robertson et al. 2013

%https://ui.adsabs.harvard.edu/abs/2013ApJ...768...71R/abstract \\

%Nakajima et al. (2018)

%https://ui.adsabs.harvard.edu/abs/2018MNRAS.477.2098N/abstract \\

%Kennicutt (1998)

%https://ui.adsabs.harvard.edu/abs/1998ARA\%26A..36..189K/abstract \\

%Worseck et al. (2014)

%https://ui.adsabs.harvard.edu/abs/2014MNRAS.445.1745W/abstract




